VersiCode: Towards Version-controllable Code Generation

Large Language Models (LLMs) have made tremendous strides in code generation, but existing research fails to account for the dynamic nature of software development, marked by frequent library updates. This gap significantly limits LLMs' deployment in realistic settings. In this paper, we propose two novel tasks aimed at bridging this gap: version-specific code completion (VSCC) and version-aware code migration (VACM). In conjunction, we introduce VersiCode, a comprehensive Python dataset specifically designed to evaluate LLMs on these two tasks, together with a novel evaluation metric, Critical Diff Check (CDC@1), which assesses code generation against evolving API requirements. We conduct an extensive evaluation on VersiCode, which reveals that version-controllable code generation is indeed a significant challenge, even for GPT-4o and other strong frontier models. We believe the novel tasks, dataset, and metric open up a new, important research direction that will further enhance LLMs' real-world applicability. The code and resources can be found at https://github.com/wutong8023/VersiCode.

==> sections/2_old_dataset_construction.tex <==
\section{VersiCode: A Benchmark for Version-controllable Code Generation}
\label{sect:dataset}
VersiCode is a large-scale code generation benchmark dataset focusing on evolving library dependencies. We propose two tasks to simulate real-world applications: version-specific code completion and version-aware code editing, incorporating version information into code generation constraints.
% 
First, we discuss data curation, preprocessing of noisy code snippets and FAQs into organized metadata (Section~\ref{subsect:data_curation}). Based on this metadata, we describe the task design and quality control process (Section~\ref{subsect:task_design}). We then address tagging API lifespan features per library version (Section~\ref{subsect:back_compatib}). Finally, we provide data statistics for VersiCode and discuss future dataset extensions (Section~\ref{subsect:data_statist}).

\subsection{Dataset Curation and Collection}
\label{subsect:data_curation}
% \tong{TODO4: shorten this section and formally define metadata.}
As shown in Figure~\ref{fig:preprocess}, we first collected permissively licensed Python repositories from GitHub that serve as the source code for Python libraries. These repositories are ranked by their popularity (as indicated by their collected stars). Using the list of popular libraries, we gathered data from three sources for each library:
(1) Library Source Code: We collected all available versions of the library source code from GitHub, verifying with PyPI to ensure that the collected versions are formally released and can be installed via pip. From the library source code, we extracted official usage examples for each API from the docstrings.
(2) Downstream Application Code: Given Python's popularity in scientific programming, we collected the source code from top-tier research papers over 10 years as downstream applications. These applications are valuable due to being lightweight yet self-consistent, diverse in their topics, and tagged release timelines associated with publishing venues. Given the time span, this data source implicitly includes evolving libraries.
(3) Stack Overflow: Using the library names as queries, we collected FAQ data from Stack Overflow, which provides real user queries and diverse user answers. We filtered the data to include only those queries that explicitly mention the versions of the libraries used, using heuristic rules, refer to Appendix~\ref{apd:annotation}.

Given the high diversity and varied quality of the collected raw data, we adopted a hybrid annotation approach involving both human experts and LLMs, such as ChatGPT. (1) Library Source Code: The library version is concrete and explicitly available, but example usage varies across libraries and versions. We used an LLM with in-context learning to help extract example code from docstrings, preparing the library version and code snippets. (2) Downstream Applications: The version can easily be extracted from configuration files, typically named ``requirements.txt''. We carefully filtered out Python files that are too long, do not mention the library version, or fail to compile. (3) Stack Overflow: Given the diversity of the questions, we designed strict heuristic rules to preliminarily annotate the library name, version, and corresponding Python code snippets mentioned in answers. We then distributed the pre-annotated data to six qualified human experts for verification and correction, ensuring the library version and code snippets are ready as well.
% 
With all pairs of library versions and code snippets, we employed ChatGPT with in-context learning to generate descriptions of the functionality for each code snippet. Each pair is wrapped in well-organized metadata.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth, bb=0 0 645 210]{figure/preprocess.pdf}
    \caption{The preprocessing pipeline to obtain metadata, structured as n-gram tuple of $<$library name, version, functionality description, code snippet$>$.\label{fig:preprocess}}
\end{figure*}

\subsection{Task Design for Version-controllable Code Generation}
\label{subsect:task_design}
As shown in Figure~\ref{fig:postprocess}, we define each meta-instance $m_i = [l_i; v_i; d_i; c_i] \in \mathcal{M} $, where $ l $, $ v $, $ d $, and $ c $ represent the library name, version, functionality description, and code snippet, respectively. We then design the following two version-controllable code generation tasks:

\noindent\textbf{Version-Specific Code Completion (VSCC)}: Given a meta-instance $ m_i $, the input is $ x = [l_i; v_i; d_i; c'_i] $, where $ c'_i $ is the code snippet $ c_i $ with selective masking, replacing the library- and version-sensitive contents with a special token. Depending on the length of the masked contents, the special token is defined as ``[token-mask]'', ``[line-mask]'', or ``[block-mask]'', reflecting code completion on different granularity levels. The output $ y $ is the masked content, typically containing function names or variables.

\noindent\textbf{Version-Aware Code Editing (VACE)}: Given a pair of meta-instances $ (m_i, m_j | l_i == l_j, d_i == d_j, v_i \neq v_j) $, the input $ x = [l_i; v_i; d_i; c_i; v_j] $, and the output $ y = c_j $. Note that version editing may require refactoring of the code structure, making it difficult to format as detailed as in token-level or line-level completion. Additionally, depending on the numerical relationship between $ v_i $ and $ v_j $, various scenarios arise, such as editing from an old version to a new version, or vice versa.

% Options selection

\subsection{Lifespan Tagging of APIs}
% \label{subsect:back_compatib}
Consider an API $a$ added to the library $L$ in version $V_s$ and deprecated in version $V_e$, and is active in the intermediate version $V_m$ where $s \leq m \leq e$. We refer to the interval $[s,e)$ as the \emph{lifespan} of $a$. To analyze model performance in detail, we assessed how up-to-date each LLM was concerning newly added or deprecated APIs per version. We compared the source code between any two consecutive versions of each library to detect changes in API or method names. Based on the detection results, we labeled the datasets obtained from the library source code as follows: ``addition'' indicates an API newly added in the current version and still applicable in subsequent versions; ``deprecation'' indicates the current version is the last usable version for the API; and ``general'' indicates the API usage method is inherited from the previous version. 


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth, bb=0 0 780 246]{figure/postprocess.pdf}
    \caption{\tong{TODO2: change the motivation example.} The post-processing pipeline transforms metadata into specific tasks and the running example per task: (left) Leveraging pairs of metadata that share the same functionality but different library versions to construct block-level code editing instances; (right) Utilizing each metadata sample, masking version-sensitive content to create multi-granularity code completion instances.\label{fig:postprocess}}
    
\end{figure*}


\subsection{Dataset Statistics, Scope, and Future Extensions}
\label{subsect:data_statist}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[t]
% \centering
% \caption{Comparison between VersiCode and other code editing datasets, with VersiCode standing out as the largest annotated dataset specifically tailored for version adaptation.\label{tab:com_edit}}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% \textbf{Benchmark} & \textbf{Source} & \textbf{Language} & \textbf{Samples} & \textbf{Editing Task} & \textbf{Granularity} & \textbf{Collection Time} & \textbf{Annotation}                 \\ \midrule
% \multicolumn{1}{c}{Defects4J~\cite{JustJE14}}                                                             & \multicolumn{1}{c}{Open Source Programs}              & \multicolumn{1}{c}{Java}         & \multicolumn{1}{c}{357}       & \multicolumn{1}{c}{Debug}            & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2014} & \multicolumn{1}{c}{None}  \\ \midrule
% \multicolumn{1}{c}{QuixBugs~\cite{LinKCS17}}                                                              & \multicolumn{1}{c}{Quixey Challenges}                 & \multicolumn{1}{c}{Python, Java} & \multicolumn{1}{c}{40}        & \multicolumn{1}{c}{Debug}            & \multicolumn{1}{c}{Line-Level}               & \multicolumn{1}{c}{2017} & \multicolumn{1}{c}{Human} \\ \midrule
% \multicolumn{1}{c}{CoST~\cite{Zhu0R22}}                                                                   & \multicolumn{1}{c}{GeeksForGeeks}                     & \multicolumn{1}{c}{Multi(=7)}    & \multicolumn{1}{c}{132,046}   & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Line-Level, Block-Level}  & \multicolumn{1}{c}{2022} & \multicolumn{1}{c}{None}  \\ \midrule
% \multicolumn{1}{c}{XLCoST~\cite{abs-2206-08474}} & \multicolumn{1}{c}{GeeksForGeeks}                     & \multicolumn{1}{c}{Multi(=8)}    & \multicolumn{1}{c}{1,083,000} & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Line-Level, Block-Level}  & \multicolumn{1}{c}{2022} & \multicolumn{1}{c}{None}  \\ \midrule
% \multicolumn{1}{c}{InstructCoder~\cite{abs-2310-20329}}                                                   & \multicolumn{1}{c}{Github}                            & \multicolumn{1}{c}{Python}       & \multicolumn{1}{c}{114,000}   & \multicolumn{1}{c}{Code Refinement}  & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{LLM}   \\ \midrule
% \multicolumn{1}{c}{MultilingualTrans~\cite{YanTLCW23}}                                                    & \multicolumn{1}{c}{Programming Sites}                 & \multicolumn{1}{c}{Multi(=8)}    & \multicolumn{1}{c}{30,419}    & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{None}  \\ \midrule
% \multicolumn{1}{c}{NicheTrans~\cite{YanTLCW23}}                                                           & \multicolumn{1}{c}{Programming Sites}                 & \multicolumn{1}{c}{Multi(>8)}    & \multicolumn{1}{c}{236,468}   & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{None}  \\ \midrule
% \multicolumn{1}{c}{LLMTrans~\cite{YanTLCW23}}                                                             & \multicolumn{1}{c}{Hand-Written}                      & \multicolumn{1}{c}{Multi(=8)}    & \multicolumn{1}{c}{350}       & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{Human} \\ \midrule
% \multicolumn{1}{c}{Avatar~\cite{AhmadTCC23}}                                                              & \multicolumn{1}{c}{Programming Sites}                 & \multicolumn{1}{c}{Python, Java} & \multicolumn{1}{c}{62,520}    & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{None}  \\ \midrule
% \multicolumn{1}{c}{G-TransEval~\cite{JiaoYLQGS23}}                                                        & \multicolumn{1}{c}{Existing benchmark, GeeksForGeeks} & \multicolumn{1}{c}{Multi(=5)}    & \multicolumn{1}{c}{400}       & \multicolumn{1}{c}{Code Translation} & \multicolumn{1}{c}{Token-Level, Block-Level} & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{Human} \\ \midrule
% \multicolumn{1}{c}{EvalGPTFix~\cite{abs-2310-08879}}                                                      & \multicolumn{1}{c}{AtCoder}                           & \multicolumn{1}{c}{Java}         & \multicolumn{1}{c}{151}       & \multicolumn{1}{c}{Debug}            & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2023} & \multicolumn{1}{c}{Human} \\ \midrule
% \multicolumn{1}{c}{DebugBench~\cite{abs-2401-04621}}                                                      & \multicolumn{1}{c}{LeetCode}                          & \multicolumn{1}{c}{Multi(=3)}    & \multicolumn{1}{c}{4,253}     & \multicolumn{1}{c}{Debug}            & \multicolumn{1}{c}{Block-Level}              & \multicolumn{1}{c}{2024} & \multicolumn{1}{c}{LLM}   \\ \midrule
% \textbf{VersiCode}                                                                                                   & Github                                                 & Python                            & 98,692                         & Version Adaptation                    & Block-Level                                   & 2024                      & LLM                        \\ \bottomrule
% \end{tabular}
% }
% % \end{table}

\noindent\textbf{Dataset Statistics}: We present the statistics of VersiCode in Table~\ref{tab:brief_data}, using the NLTK~\footnote{\url{https://www.nltk.org/}} tokenizer to compute the number of tokens. 
As shown in Table~\ref{tab:com_edit}, we also provide a comparison between VersiCode and other code editing datasets. See Appendix~\ref{subapd:completion} for the comparison between VersiCode and other code completion datasets.

\noindent\textbf{Scope}: VersiCode supports version-specific code completion at the token, line, and block levels, enabling developers to navigate through version variations effortlessly. It also facilitates block-level version-aware code editing, empowering users to make precise modifications tailored to requirements of each version. 
% 
The collected metadata also serves as a valuable resource for potential customized task modifications, aiding in fine-tuning workflows and enhancing model training for optimal performance.

\begin{wraptable}{r}{0.53\textwidth}% "l" for left and "0.5\textwidth" for the width of the image
\centering
\vspace{-5mm}
\caption{Data statistics of VersiCode.}\label{tab:brief_data}
\vspace{2mm}
\resizebox{.53\textwidth}{!}{
\begin{tabular}{@{}cccccc@{}}
\toprule
\# Num. of Libraries & \multicolumn{5}{c}{300}                                                                                                                                  \\ \midrule
\# Num. of Versions  & \multicolumn{5}{c}{2,207}                                                                                                                                \\ \midrule
\# Size of Metadata & \multicolumn{5}{c}{11,268}                                                                                                                               \\ \midrule
\# Task Type         & \multicolumn{3}{c}{Completion}                                                        & \multicolumn{1}{c}{Editing (old to new)} & Editing (new to old) \\ \cmidrule(r){1-1}\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
\# Granularity       & \multicolumn{1}{c}{Token}  & \multicolumn{1}{c}{Line}   & \multicolumn{1}{c}{Block} & \multicolumn{1}{c}{Block}                & Block                \\ \midrule
\# Avg. Input Token  & \multicolumn{1}{c}{1,233}  & \multicolumn{1}{c}{1,213}  & \multicolumn{1}{c}{44}    & \multicolumn{1}{c}{115}                  & 116                  \\ \midrule
\# Avg. Output Token & \multicolumn{1}{c}{1}      & \multicolumn{1}{c}{9}      & \multicolumn{1}{c}{77}    & \multicolumn{1}{c}{70}                   & 69                   \\ \midrule
\# Num. of Instances & \multicolumn{1}{c}{13,532} & \multicolumn{1}{c}{13,530} & \multicolumn{1}{c}{1,618} & \multicolumn{1}{c}{49,346}               & 49,346               \\ \bottomrule
\end{tabular}}
\vspace{-3mm}
\end{wraptable}

\noindent\textbf{Future Extension}: VersiCode primarily supports Python, but we have also made efforts to extend it to multiple languages. Refer to the Appendix~\ref{subapd:data_statis} for comprehensive data statistics and initial multi-language evaluation results. Given the rapid evolution of software technologies, continued effort to further automate the curation pipeline and maintenance of VersiCode is needed.




==> sections/3_old_experiments.tex <==
\section{Experiments}
\tong{TODO6: change it into 3-stage studies: 1) including token-level and time analyses. 2) block-level completion, and metric analysis. 3) code migration analysis.}

We undertake experiments to investigate the following research questions:
\begin{enumerate}[noitemsep,nolistsep]
\item What is the quality and difficulty of VersiCode, particularly in comparison to related datasets and among diverse data sources?
\item What is the current proficiency of codeLLMs in generating version-controllable code, considering comparisons among multiple-granularity completions, for both code completion and code editing?
\item What is the timeliness of LLMs' programming knowledge in code generation, with a focus on model performance categorized by year over the past decade?
\end{enumerate}


\subsection{Implementation Details}
\label{subsect:imple_detail}

\noindent\textbf{Models}: 
We benchmarked VersiCode against popular open-domain LLMs and dedicated code-LLMs, including variant families such as GPT~\cite{abs-2303-08774,gpt35,gpt4o}, LLaMa~\cite{abs-2307-09288}, Mistral~\cite{abs-2310-06825}, CodeLLaMa~\cite{abs-2308-12950}, CodeQwen~\cite{qwen}, CodeGemma~\cite{codegemma_2024}, StarCoder~\cite{abs-2402-19173}, Deepseek-Coder~\cite{abs-2401-14196}, and WizardCoder~\cite{abs-2306-08568}. For smaller open-source models (e.g., < 20B parameters), we downloaded them from HuggingFace~\footnote{\url{https://huggingface.co/models}} and deployed them locally for inference. For larger models, such as LLaMa3 70B~\cite{llama3modelcard} and GPT-4o~\cite{gpt4o}, we used their online APIs~\footnote{\url{https://together.ai}}~\footnote{\url{https://openai.com/}} for inference.

\noindent\textbf{Baseline Dataset}: To assess the difficulty of VersiCode, we compared it with two well-known code generation datasets, HumanEval~\cite{LiuXW023} and MBPP~\cite{jiang2024survey}, and observed the overall performance of models. HumanEval~\cite{LiuXW023} measures functional correctness in synthesizing programs from docstrings with 164 original problems, resembling simple software interview questions. MBPP~\cite{abs-2108-07732}, with about 1,000 crowd-sourced Python problems for entry-level programmers, covers programming fundamentals and standard library functionality, including task descriptions, code solutions, and three automated test cases for each problem. We also collected the evaluation results for their upgraded versions HumanEval+~\cite{LiuXW023} and MBPP+~\cite{LiuXW023}. Please refer to Appendix~\ref{subapd:main} for details.

\noindent\textbf{Data Preparation}: As introduced in Section~\ref{subsect:task_design}, we designed two types of version-controllable code generation tasks: version-specific code completion and version-aware code editing. The task granularities are categorized into token-level, line-level, and block-level to control difficulty and simulate different application scenarios. To better understand model performance, each instance in VersiCode is also tagged with the following: (1) data source, which includes library source code, downstream applications, and Stack Overflow (see Section~\ref{subsect:data_curation}); (2) feature type, including addition, deprecation, and general (see Section~\ref{subsect:back_compatib}); (3) release time, i.e.\ the timestamp from GitHub and Stack Overflow); and (4) considering code editing instances constructed from pairs of metadata, the differences between source and target code versions result in various situations, such as updates from an older version to a newer version or vice versa. Additionally, we categorized versions according to version patterns, for example, treating torch v1.0.0 as a major version and torch v1.3.1 as a minor version, to identify combinations of major and minor version editing cases.
% 
These tags allow us to filter the evaluation dataset and gain sharper insights into model performance.

\noindent\textbf{Evaluation Metrics}:
We use the following evaluation metrics for each task granularity:
% 
(1) \textbf{Pass@$k$} for token-level generation~\cite{abs-2107-03374}: For this metric, we generate $n \geq k$ samples per instance (with $n=100$ and $k\in\{1, 3, 10\}$ for our experiments). We count the number of correct samples $c \leq n$ judged by exact matching. Pass@$k$ is defined as the average performance over the task, calculated as $\mathbb{E} \left[ 1 - \frac{{\binom{n-c}{k}}} {\binom{n}{k}} \right]$.
% 
(2) \textbf{Identifier Sequence Match (ISM@$n$)} and \textbf{Prefix Match (PM@$n$)} for line-level generation~\cite{abs-2306-10763}: These metrics measure how closely the generated sequences match the ground truth. For block-level generation, we adopt the average performance over lines. Following the setup in Agrawal et al.~\cite{abs-2306-10763}, we generate $n=6$ independent samples per instance.

\subsection{Results and Analysis}
\label{subsect:analysis_exp}

\begin{figure*}[t]
    \includegraphics[width=1.0\linewidth, bb=0 0 960 250]{figure/main_result.pdf}
    \caption{Pass@1 results for token-level code completion from VersiCode: (a1) comparison with existing benchmark datasets, (a2) performance grouped by data sources, and (b) performance grouped by API lifespan features.\label{fig:main}}
\end{figure*}


\noindent\textbf{Even token-level code completion is challenging.}
We present the pass@1 results of token-level code completion for LLMs on VersiCode, sorted by release time (see Figure~\ref{fig:main}-a1, highlighted in green). When compared to the Pass@1 results on HumanEval (in blue) and MBPP (in orange), all models perform significantly worse on VersiCode (in green). This result indicates the difficulty in disambiguating and recalling version-specific library usage. It is worth noting that the larger and latest models, such as GPT-4o (M13) and LLaMA3-70B (M12), achieve significantly better performance than the other models (See Appendix~\ref{subapd:ea} for the error analysis of GPT-4o.). However, the performance gap with HumanEval and MBPP is still large, with at least 15 points. Thus, for the simplest token-level completion task, state-of-the-art LLMs struggle to achieve satisfactory performance. % might demonstrate the verifiable quality of the proposed dataset.

\noindent\textbf{Differences in LLM performance across different data sources.}
We present the Pass@1 results, categorized by data sources, of token-level code completion for LLMs on VersiCode in Figure~\ref{fig:main}-a2. Comparing these three data sources, most models perform much better on Stack Overflow than on the other two, especially the source code from downstream applications. This result may be due to the high diversity in downstream applications, which requires a strong ability to tackle them. It may also suggest that Stack Overflow is highly represented in the pre-training data of LLMs, hence a greater chance of data leakage. Similar to Figure~\ref{fig:main}-a1, the outliers are still GPT-4o (M13) and LLaMA3-70B (M12), which excel in dealing with downstream applications increasing the likelihood of models memorizing specific content. Please refer to Appendix~\ref{subapd:main} for full numeric results.


% Analysis 1
\noindent\textbf{Challenges in casual intermediate library versions.}
We present the token-level Pass@1 results categorized by lifespan features: addition (in blue), deprecation (in orange), and general (referring to intermediate versions; in green) for the token-level code completion task (see Figure~\ref{fig:main}-b). Most models perform well in the cases of addition and deprecation due to newly added or deprecated APIs, as these versions are likely emphasized in documentation or by the community. However, most models struggle with reasoning and adapting to intermediate versions. When viewed alongside Figure~\ref{fig:main}-a2, it is evident that models such as LLaMA3-70B perform better in downstream applications and are also good at intermediate versions, benefiting from the diversity of use cases.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\vspace{2mm}
\caption{Evaluation of multi-granularity version-specific code completion, and version-adapted code editing in both ``old $\mapsto$ new'' and ``new $\mapsto$ old'' scenarios.\label{tab:granularity}}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule

\multirow{4}{*}{\textbf{Model}}          & \multicolumn{7}{c}{\textbf{Code Completion}} & \multicolumn{2}{c}{\textbf{Code Editing} (old $\mapsto$ new)}   & \multicolumn{2}{c}{\textbf{Code Editing} (new $\mapsto$ old)}   \\ 
\cmidrule(lr){2-8} \cmidrule(lr){9-12} 
                                & \multicolumn{3}{c}{Token-level} & \multicolumn{2}{c}{Line-level} & \multicolumn{2}{c}{Block-level}                & \multicolumn{2}{c}{Block-level}                & \multicolumn{2}{c}{Block-level}                \\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12}  
                                & Pass@1 & Pass@3 & Pass@10 & ISM@6 & PM@6 & ISM@6 & PM@6 & ISM@6 & PM@6 & ISM@6 & PM@6 \\ \midrule
DeepSeek-Coder-7B-Instruct-V1.5~\cite{abs-2401-14196} & \multicolumn{1}{c}{15.71}  & \multicolumn{1}{c}{21.72}  & \multicolumn{1}{c}{27.84}   & \multicolumn{1}{c}{35.59} & \multicolumn{1}{c}{22.53} & \multicolumn{1}{c}{0}     & 0     & \multicolumn{1}{c}{45.41}       & 36.44      & \multicolumn{1}{c}{40.25}       & 28.89      \\ \midrule
CodeLlama-13B-Instruct~\cite{abs-2308-12950}          & \multicolumn{1}{c}{13.5}   & \multicolumn{1}{c}{20.29}  & \multicolumn{1}{c}{26.87}   & \multicolumn{1}{c}{29.22} & \multicolumn{1}{c}{16.69} & \multicolumn{1}{c}{4.34}  & 3.12  & \multicolumn{1}{c}{39.17}       & 27.94      & \multicolumn{1}{c}{39.12}       & 26.17      \\ \midrule
StarCoder2-15B~\cite{abs-2402-19173}                  & \multicolumn{1}{c}{14.55}  & \multicolumn{1}{c}{21.35}  & \multicolumn{1}{c}{27.59}   & \multicolumn{1}{c}{20.37} & \multicolumn{1}{c}{12.46} & \multicolumn{1}{c}{1.36}  & 0.79  & \multicolumn{1}{c}{35.59}       & 26.72      & \multicolumn{1}{c}{41.41}       & 27.64      \\ \midrule
CodeGemma-7B~\cite{codegemma_2024}                    & \multicolumn{1}{c}{13.28}  & \multicolumn{1}{c}{18.79}  & \multicolumn{1}{c}{24.09}   & \multicolumn{1}{c}{5.2}   & \multicolumn{1}{c}{2.57}  & \multicolumn{1}{c}{0.37}  & 0.22  & \multicolumn{1}{c}{9.16}        & 4.12       & \multicolumn{1}{c}{9.72}        & 5.28       \\ \midrule
GPT-3.5-Turbo~\cite{gpt35}          & \multicolumn{1}{c}{37.59}  & \multicolumn{1}{c}{44.62}  & \multicolumn{1}{c}{51.17}   & \multicolumn{1}{c}{49.19} & \multicolumn{1}{c}{32.85} & \multicolumn{1}{c}{40.28} & 27.57 & \multicolumn{1}{c}{45.96}       & 36.8       & \multicolumn{1}{c}{46.96}       & 35.06      \\ \midrule
Llama-3-70B-Chat~\cite{llama3modelcard}               & \multicolumn{1}{c}{47.55}  & \multicolumn{1}{c}{52.42}  & \multicolumn{1}{c}{55.77}   & \multicolumn{1}{c}{49.62} & \multicolumn{1}{c}{33.14} & \multicolumn{1}{c}{57.68} & 41.47 & \multicolumn{1}{c}{33.37}       & 23.51      & \multicolumn{1}{c}{42.94}       & 29.36      \\ \midrule
GPT-4o~\cite{gpt4o}                & \multicolumn{1}{c}{70.44}  & \multicolumn{1}{c}{74.27}  & \multicolumn{1}{c}{77.27}   & \multicolumn{1}{c}{69.44} & \multicolumn{1}{c}{58.95} & \multicolumn{1}{c}{64.73} & 50.48 & \multicolumn{1}{c}{54.72}       & 45.04      & \multicolumn{1}{c}{55.36}       & 52.33      \\ \bottomrule

\end{tabular}}
\end{table}

\noindent\textbf{Reduced context increases error risk in code generation.}
Based on the token-level code completion performance of each model, we selected the top models for further analysis. We present the multi-granularity comparison in Table~\ref{tab:granularity}. When comparing the performance between line-level and block-level code completion, we can observe that smaller models tend to fail more frequently at generating correct code in block-level completion, due to less code context and the requirement to generate more content, which aligns with our intuition. Note that the results shown here have been filtered by \emph{grammar verification}, a post-generation validation step that only counts code that successfully compiles in Python. If we remove grammar verification, the overall performance of block-level completion in Table~\ref{tab:wogrammar} (Appendix~\ref{subapd:wo_verify}) is comparable to line-level completion in Table~\ref{tab:granularity}. This suggests that while the models can predict code-style content, they cannot guarantee correct programming grammar.


\noindent\textbf{The context code in another version is still helpful, but its benefits are limited.}
The comparison between block-level code completion and block-level code editing is shown in Table~\ref{tab:granularity}. There is a significant improvement across most models, except for LLaMA3-70B and GPT4-o. When provided with code in another version as context (i.e.\ in the code editing task), these models can generate correct code with a much higher success rate. However, a bottleneck is evident in LLaMA3-70B and GPT4-o, where the code context hinders their performance compared to code completion.


\noindent\textbf{Major version matters in version-aware code editing.}
As shown in Table~\ref{tab:granularity}, ``old to new'' editing and ``new to old'' demonstrate similar performance among models. 
% 
As shown in Figure~\ref{tab:varedit}, we categorize editing instances according to their source and target versions, distinguishing between major and minor versions. 
It's evident that when the major version serves as the source, the model's editing performance is inferior compared to other scenarios.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\caption{Performance of the model's editing capabilities, influenced by transitions between source and target versions, such as shifts from major to minor versions or vice versa.\label{tab:varedit}}
\resizebox{.8\textwidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}                       & \multicolumn{2}{c}{\textbf{Major$\mapsto$Major}} & \multicolumn{2}{c}{\textbf{Major$\mapsto$Minor}} & \multicolumn{2}{c}{\textbf{Minor$\mapsto$Major}} & \multicolumn{2}{c}{\textbf{Minor$\mapsto$Minor}} \\ \cmidrule(l){2-9} 
                                                      & ISM@6                   & PM@6                   & ISM@6                   & PM@6                   & ISM@6                   & PM@6                   & ISM@6                   & PM@6                   \\ \midrule
DeepSeek-Coder-7B-Instruct-V1.5~\cite{abs-2401-14196} & 12.83                   & 11.10                  & 23.73                   & 18.91                  & 30.71                   & 22.97                  & 36.29                   & 21.82                  \\ \midrule
CodeLlama-13B-Instruct~\cite{abs-2308-12950}          & 15.4                    & 14.2                   & 23.07                   & 18.29                  & 29.10                    & 20.65                  & 34.09                   & 20.36                  \\ \midrule
StarCoder2-15B~\cite{abs-2402-19173}                  & 14.94                   & 13.40                   & 19.90                    & 14.87                  & 24.74                   & 16.99                  & 35.10                    & 21.91                  \\ \midrule
CodeGemma-7B~\cite{codegemma_2024}                    & 7.71                    & 5.89                   & 7.10                     & 6.03                   & 6.00                       & 3.54                   & 13.45                   & 7.93                   \\ \midrule
GPT-3.5-Turbo~\cite{gpt35}          & 14.47                   & 12.40                   & 24.57                   & 20.60                   & 32.07                   & 25.20                   & 39.57                   & 25.57                  \\ \midrule
Llama-3-70B-Chat~\cite{llama3modelcard}               & 15.50                    & 14.10                   & 20.47                   & 17.00                     & 21.46                   & 16.35                  & 32.40                    & 19.77                  \\ \midrule
GPT-4o~\cite{gpt4o}                 & 26.21                   & 24.60                   & 41.39                   & 37.23                  & 50.01                   & 44.20                   & 59.55                   & 47.40                   \\ \bottomrule
\end{tabular}
}
\end{table}


% Analysis 4
% \subsubsection{(Optional) Multi-Language Extension}

% \noindent\textbf{Objective}: If initial experiments are successful, extend the evaluation to include multiple programming languages to assess the dataset's broader applicability.

% \noindent\textbf{Languages}: Potential addition of JavaScript, Java, or C++.

% \noindent\textbf{Metrics}: Cross-language version control accuracy, adaptability of models across different syntaxes and APIs.
\begin{figure}[t]
    \centering
    % , bb=0 0 960 540
    \includegraphics[width=1.0\textwidth,bb=0 0 945 300]{figure/time.pdf}
    \caption{Pass@1 performance for token-level code completion, grouped by year (2015-2023), with a histogram of data distribution for each year.\label{fig:time_analysis}}
\end{figure}
% Error Analysis
\noindent\textbf{The programming knowledge of LLMs, particularly regarding version-specific information, is surprisingly outdated.}
In Figure~\ref{fig:time_analysis} we present the Pass@1 performance for token-level code completion, grouped by year, covering 2015-2023. Additionally, we show the histogram of data distribution for each year. To ensure precise timestamps and minimize noise, we only used instances collected from library source code. As shown in Figure~\ref{fig:time_analysis}-a we can observe a general trend: the later the time, the worse the models' performance. This is counter-intuitive compared to temporal knowledge question answering~\cite{abs-2402-16797}, where performance initially increases before declining. We further filtered for ``deprecation'' (Figure~\ref{fig:time_analysis}-b) and ``addition'' (Figure~\ref{fig:time_analysis}-c) to identify version-sensitive cases. While the sparsity of data decreases confidence in results, in both cases, we can observe a consistent decreasing trend over time. This suggests that LLMs have outdated programming knowledge, highlighting the need for rapid adaptation to newer libraries and APIs.




==> sections/7_limitation.tex <==
\section{Limitation}
\label{sec:limit}
% editing schema
While the construction of VersiCode involved LLM-generated annotations and a partially automated pipeline, it still requires a certain amount of human annotation work for quality control. Fully automating the dataset curation and maintenance process~\cite{abs-2402-14652} requires further development. This capability is especially important given the potential risk of dataset contamination~\cite{LiF24} and the ever-evolving nature of libraries and APIs~\cite{LamotheGS22}.
% 
Another limitation of the current VersiCode dataset is its handling of multiple programming languages. While we have conducted annotations on Java, JavaScript, and C\# from Stack Overflow, as shown in Appendix~\ref{subapd:data_statis} and ~\ref{subapd:mla}, the data size for these languages is not comparable to Python. More effort, similar to that invested in constructing the Python version of VersiCode, is required for other languages.
% 
The final limitation of the current VersiCode dataset is the simplicity of the editing scheme~\cite{JiaoYLQGS23}, improving which may bridge the gap between code generation and real-world software engineering tasks. 


==> sections/8_reproducibility_ethics_statement.tex <==
\section{Reproducibility Statement}
We have open-sourced the VersiCode codebase, including data collection and evaluation scripts, along with the data (raw corpus, metadata, and manually verified test cases). 
% We've also provided documentation and a project website. x
To ensure reproducibility, data subsets from sections 3 to 5 are separately packaged in the supplementary files, and
the evaluation prompts and parameter settings are included in Appendix~\ref{apd:evaluation_details}.



% \section{Ethics statement}
% \tong{data filtering}

==> table/brief_data_statis.tex <==
\begin{wraptable}{r}{0.53\textwidth}% "l" for left and "0.5\textwidth" for the width of the image
\centering
\vspace{-5mm}
\caption{Data statistics of VersiCode.}\label{tab:brief_data}
\vspace{2mm}
\resizebox{.53\textwidth}{!}{
\begin{tabular}{@{}cccccc@{}}
\toprule
\# Num. of Libraries & \multicolumn{5}{c}{300}                                                                                                                                  \\ \midrule
\# Num. of Versions  & \multicolumn{5}{c}{2,207}                                                                                                                                \\ \midrule
\# Size of Metadata & \multicolumn{5}{c}{11,268}                                                                                                                               \\ \midrule
\# Task Type         & \multicolumn{3}{c}{Completion}                                                        & \multicolumn{1}{c}{Editing (old to new)} & Editing (new to old) \\ \cmidrule(r){1-1}\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
\# Granularity       & \multicolumn{1}{c}{Token}  & \multicolumn{1}{c}{Line}   & \multicolumn{1}{c}{Block} & \multicolumn{1}{c}{Block}                & Block                \\ \midrule
\# Avg. Input Token  & \multicolumn{1}{c}{1,233}  & \multicolumn{1}{c}{1,213}  & \multicolumn{1}{c}{44}    & \multicolumn{1}{c}{115}                  & 116                  \\ \midrule
\# Avg. Output Token & \multicolumn{1}{c}{1}      & \multicolumn{1}{c}{9}      & \multicolumn{1}{c}{77}    & \multicolumn{1}{c}{70}                   & 69                   \\ \midrule
\# Num. of Instances & \multicolumn{1}{c}{13,532} & \multicolumn{1}{c}{13,530} & \multicolumn{1}{c}{1,618} & \multicolumn{1}{c}{49,346}               & 49,346               \\ \bottomrule
\end{tabular}}
\vspace{-3mm}
\end{wraptable}

==> table/granularity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\vspace{2mm}
\caption{Evaluation of multi-granularity version-specific code completion, and version-adapted code migration in both ``old $\mapsto$ new'' and ``new $\mapsto$ old'' scenarios.\label{tab:granularity}}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule

\multirow{4}{*}{\textbf{Model}}          & \multicolumn{7}{c}{\textbf{Code Completion}} & \multicolumn{2}{c}{\textbf{Code Editing} (old $\mapsto$ new)}   & \multicolumn{2}{c}{\textbf{Code Editing} (new $\mapsto$ old)}   \\ 
\cmidrule(lr){2-8} \cmidrule(lr){9-12} 
                                & \multicolumn{3}{c}{Token-level} & \multicolumn{2}{c}{Line-level} & \multicolumn{2}{c}{Block-level}                & \multicolumn{2}{c}{Block-level}                & \multicolumn{2}{c}{Block-level}                \\ \cmidrule(l){2-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12}  
                                & Pass@1 & Pass@3 & Pass@10 & ISM@6 & PM@6 & ISM@6 & PM@6 & ISM@6 & PM@6 & ISM@6 & PM@6 \\ \midrule
DeepSeek-Coder-7B-Instruct-V1.5~\cite{abs-2401-14196} & \multicolumn{1}{c}{15.71}  & \multicolumn{1}{c}{21.72}  & \multicolumn{1}{c}{27.84}   & \multicolumn{1}{c}{35.59} & \multicolumn{1}{c}{22.53} & \multicolumn{1}{c}{0}     & 0     & \multicolumn{1}{c}{45.41}       & 36.44      & \multicolumn{1}{c}{40.25}       & 28.89      \\ \midrule
CodeLlama-13B-Instruct~\cite{abs-2308-12950}          & \multicolumn{1}{c}{13.5}   & \multicolumn{1}{c}{20.29}  & \multicolumn{1}{c}{26.87}   & \multicolumn{1}{c}{29.22} & \multicolumn{1}{c}{16.69} & \multicolumn{1}{c}{4.34}  & 3.12  & \multicolumn{1}{c}{39.17}       & 27.94      & \multicolumn{1}{c}{39.12}       & 26.17      \\ \midrule
StarCoder2-15B~\cite{abs-2402-19173}                  & \multicolumn{1}{c}{14.55}  & \multicolumn{1}{c}{21.35}  & \multicolumn{1}{c}{27.59}   & \multicolumn{1}{c}{20.37} & \multicolumn{1}{c}{12.46} & \multicolumn{1}{c}{1.36}  & 0.79  & \multicolumn{1}{c}{35.59}       & 26.72      & \multicolumn{1}{c}{41.41}       & 27.64      \\ \midrule
CodeGemma-7B~\cite{codegemma_2024}                    & \multicolumn{1}{c}{13.28}  & \multicolumn{1}{c}{18.79}  & \multicolumn{1}{c}{24.09}   & \multicolumn{1}{c}{5.2}   & \multicolumn{1}{c}{2.57}  & \multicolumn{1}{c}{0.37}  & 0.22  & \multicolumn{1}{c}{9.16}        & 4.12       & \multicolumn{1}{c}{9.72}        & 5.28       \\ \midrule
GPT-3.5-Turbo~\cite{gpt35}          & \multicolumn{1}{c}{37.59}  & \multicolumn{1}{c}{44.62}  & \multicolumn{1}{c}{51.17}   & \multicolumn{1}{c}{49.19} & \multicolumn{1}{c}{32.85} & \multicolumn{1}{c}{40.28} & 27.57 & \multicolumn{1}{c}{45.96}       & 36.8       & \multicolumn{1}{c}{46.96}       & 35.06      \\ \midrule
Llama-3-70B-Chat~\cite{llama3modelcard}               & \multicolumn{1}{c}{47.55}  & \multicolumn{1}{c}{52.42}  & \multicolumn{1}{c}{55.77}   & \multicolumn{1}{c}{49.62} & \multicolumn{1}{c}{33.14} & \multicolumn{1}{c}{57.68} & 41.47 & \multicolumn{1}{c}{33.37}       & 23.51      & \multicolumn{1}{c}{42.94}       & 29.36      \\ \midrule
GPT-4o~\cite{gpt4o}                & \multicolumn{1}{c}{70.44}  & \multicolumn{1}{c}{74.27}  & \multicolumn{1}{c}{77.27}   & \multicolumn{1}{c}{69.44} & \multicolumn{1}{c}{58.95} & \multicolumn{1}{c}{64.73} & 50.48 & \multicolumn{1}{c}{54.72}       & 45.04      & \multicolumn{1}{c}{55.36}       & 52.33      \\ \bottomrule

\end{tabular}}
\end{table}

==> table/variant_editing.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\caption{Performance of the model's editing capabilities, influenced by transitions between source and target versions, such as shifts from major to minor versions or vice versa.\label{tab:varedit}}
\resizebox{.8\textwidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}                       & \multicolumn{2}{c}{\textbf{Major$\mapsto$Major}} & \multicolumn{2}{c}{\textbf{Major$\mapsto$Minor}} & \multicolumn{2}{c}{\textbf{Minor$\mapsto$Major}} & \multicolumn{2}{c}{\textbf{Minor$\mapsto$Minor}} \\ \cmidrule(l){2-9} 
                                                      & ISM@6                   & PM@6                   & ISM@6                   & PM@6                   & ISM@6                   & PM@6                   & ISM@6                   & PM@6                   \\ \midrule
DeepSeek-Coder-7B-Instruct-V1.5~\cite{abs-2401-14196} & 12.83                   & 11.10                  & 23.73                   & 18.91                  & 30.71                   & 22.97                  & 36.29                   & 21.82                  \\ \midrule
CodeLlama-13B-Instruct~\cite{abs-2308-12950}          & 15.4                    & 14.2                   & 23.07                   & 18.29                  & 29.10                    & 20.65                  & 34.09                   & 20.36                  \\ \midrule
StarCoder2-15B~\cite{abs-2402-19173}                  & 14.94                   & 13.40                   & 19.90                    & 14.87                  & 24.74                   & 16.99                  & 35.10                    & 21.91                  \\ \midrule
CodeGemma-7B~\cite{codegemma_2024}                    & 7.71                    & 5.89                   & 7.10                     & 6.03                   & 6.00                       & 3.54                   & 13.45                   & 7.93                   \\ \midrule
GPT-3.5-Turbo~\cite{gpt35}          & 14.47                   & 12.40                   & 24.57                   & 20.60                   & 32.07                   & 25.20                   & 39.57                   & 25.57                  \\ \midrule
Llama-3-70B-Chat~\cite{llama3modelcard}               & 15.50                    & 14.10                   & 20.47                   & 17.00                     & 21.46                   & 16.35                  & 32.40                    & 19.77                  \\ \midrule
GPT-4o~\cite{gpt4o}                 & 26.21                   & 24.60                   & 41.39                   & 37.23                  & 50.01                   & 44.20                   & 59.55                   & 47.40                   \\ \bottomrule
\end{tabular}
}
\end{table}
